Automatically Planning Optimal Parallel Strategy for Large Language Models

The number of parameters in large-scale language models based on transformers is gradually increasing, and the scale of computing clusters is also growing. The technology of quickly mobilizing large amounts of computing resources for parallel computing is becoming increasingly important. In this paper, we propose an automatic parallel algorithm that automatically plans the parallel strategy with maximum throughput based on model and hardware information. By decoupling the training time into computation, communication, and overlap, we established a training duration simulation model. Based on this simulation model, we prune the parallel solution space to shorten the search time required. The multi-node experiment results show that the algorithm can estimate the parallel training duration in real time with an average accuracy of 96%. In our test, the recommendation strategy provided by the algorithm is always globally optimal.

==> table_draft.tex <==

% \begin{table}[!ht]
%     \centering
    
%     \begin{tabular}{cccc}
%     \hline
%         \textbf{Parameter} & \textbf{Value}  & \textbf{Explanation} \\ \hline
        
%         $n$  & 16      & Total number of Huawei Ascend NPUs  \\
%         $TSs$  & 256      &Total number of samples \\
%         $L$  & 32      &Total number of model layers  \\ 
%         $u$  & 2      & The size of parameters (bytes) \\
%         $g$  & 12884901888      & \makecell{Inter-server baseband bandwidth  (12GBps) }\\
%         $g'_2$  & 20      & GBps \\
%         $g_2$  & 21474836480      & Inter-server baseband bandwidth (20GBps)\\
%         $G$  & 256      & Global batch size \\
%         $s$  & 4096      & Sequence length\\
%         $h$  & 4096      & Hidden size\\ 
%         $H$  & 11008      & FNN hidden size \\
%         $V$  & 32000      &  Vocabulary size\\ 
%         $k$  & 2      & The ratio of backward computation to forward computation\\
%         \multirow{2}{*}{$U_{max}$}  & $3.13* e^{14}$      &Benchmarking computing power of 910B2 (FLOPs) \\
%         & $2.8* e^{14}$      &Benchmarking computing power of 910B3 (FLOPs) \\\hline
%     \end{tabular}
%     \caption{Parameter settings and explanations.}
%     \label{param}
% \end{table}

\begin{table*}[h]
    \centering
    
    \begin{tabular}{ccccccccccccc}
    \hline
        \textbf{\makecell{NPU\\Num}} & \textbf{t} & \textbf{b} & \textbf{steps} & \textbf{gbs} & \textbf{layers}  & \textbf{\makecell{Cmpt\\Time}} & \textbf{\makecell{$U_F$\\(TFLOPs)}} & \textbf{\makecell{Utilization\\ Rate Real}} & \textbf{\makecell{Utilization\\ Rate Est}}  & \textbf{\makecell{Error\\(\%)} }& $\omega$ & $k$  \\ \hline
        8  & 8  & 1  & 40  & 40  & 32  & 6.96  & 110.17  & 0.3520  & 0.3551  & 0.90 & 0.4196& -0.0644   \\ 
        8  & 8  & 2  & 40  & 80  & 32  & 12.43  & 123.32  & 0.3940  & 0.3874  & 1.68 &0.4196& -0.0644  \\ 
        8  & 8  & 3  & 40  & 120  & 32  & 18.37  & 125.20  & 0.4000  & 0.3981  & 0.47 &0.4196& -0.0644 \\ 
        8  & 8  & 4  & 40  & 160  & 32  & 23.92  & 128.17  & 0.4095  & 0.4035  & 1.47 &0.4196& -0.0644\\ 
        8  & 8  & 5  & 40  & 200  & 32  & 30.97  & 123.74  & 0.3953  & 0.4067  & 2.87 &0.4196& -0.0644\\ 
        4  & 4  & 1  & 40  & 40  & 32  & 11.81  & 129.84  & 0.4148  & 0.4167  & 0.46 &0.4755& -0.0587 \\ 
        4  & 4  & 2  & 40  & 80  & 32  & 21.59  & 142.03  & 0.4538  & 0.4461  & 1.69 &0.4755& -0.0587  \\ 
        4  & 4  & 3  & 40  & 120  & 32  & 32.64  & 140.90  & 0.4501  & 0.4559  & 1.27 &0.4755& -0.0587\\ 
        2  & 2  & 1  & 40  & 40  & 16 & 11.10  & 141.07  & 0.4507  & 0.4543  & 0.79 &0.4880& -0.0337 \\ 
        2  & 2  & 2  & 40  & 80  & 16  & 20.62  & 151.81  & 0.4850  & 0.4711  & 2.86 &0.4880& -0.0337 \\ 
        2  & 2  & 3  & 40  & 120  & 16  & 32.12  & 146.21  & 0.4671  & 0.4767  & 2.06 &0.4880& -0.0337 \\ 
        2  & 2  & 4  & 40  & 160  & 16  & 41.78  & 149.87  & 0.4788  & 0.4795  & 0.15 &0.4880& -0.0337\\ 
        1  & 1  & 1  & 1  & 40  & 8  & 11.18  & 145.80  & 0.4658  & 0.4672  & 0.30 &0.4894& -0.0221\\ 
        1  & 1  & 2  & 1  & 80  & 8  & 21.63  & 150.70  & 0.4815  & 0.4783  & 0.65 &0.4894& -0.0221\\ 
        1  & 1  & 3  & 1  & 120  & 8  & 32.18  & 151.93  & 0.4854  & 0.4820  & 0.69 &0.4894& -0.0221 \\ 
        1  & 1  & 4  & 1  & 160  & 8  & 43.50  & 149.86  & 0.4788  & 0.4839  & 1.06 &0.4894& -0.0221\\ \hline
    \end{tabular}
    \caption{Computing power fitting.}
    \label{computing_power}
\end{table*}
\begin{table*}[h]
    \centering
    \begin{tabular}{c|ccc|ccc|ccc|ccc}
    \hline
        \textbf{dtpb} & \textbf{\makecell{Total\\Est}} & \textbf{\makecell{Total\\Real}} & \textbf{\makecell{ACC\\(\%)}} & \textbf{\makecell{Cmpt\\Est}} & \textbf{\makecell{Cmpt\\Real}} & \textbf{\makecell{ACC\\(\%)}} & \textbf{\makecell{Comm\\Est}} & \textbf{\makecell{Comm\\Real}} & \textbf{\makecell{ACC\\(\%)}} & \textbf{\makecell{Overlap\\Est}} & \textbf{\makecell{Overlap\\Real}} & \textbf{\makecell{ACC\\(\%)}} \\ \hline
        (8 ,1 ,2 ,1)  & 18.58  & 19.14  & 97.05  & 17.18  & 17.09  & 99.49  & 1.40  & 1.78  & 78.54  & 0.00  & 0.00  & 100.00  \\ 
        (4 ,1 ,4 ,1)  & 19.32  & 20.12  & 96.02  & 17.88  & 17.62  & 98.52  & 1.44  & 2.09  & 68.86  & 0.00  & 0.00  & 100.00  \\ 
        (4 ,1 ,4 ,2)  & 19.47  & 20.24  & 96.23  & 17.30  & 17.30  & 99.98  & 2.17  & 2.65  & 81.82  & 0.00  & 0.00  & 100.00  \\ 
        (2 ,1 ,8 ,1)  & 21.01  & 21.71  & 96.81  & 19.30  & 18.90  & 97.90  & 1.71  & 2.16  & 79.31  & 0.00  & 0.00  & 100.00  \\ 
        (2 ,1 ,8 ,2)  & 22.26  & 21.90  & 97.09  & 18.67  & 18.45  & 98.81  & 2.59  & 2.83  & 91.42  & 0.00  & 0.00  & 100.00  \\ 
        (8 ,2 ,1 ,1)  & 22.37  & 23.05  & 97.07  & 17.38  & 17.11  & 98.39  & 7.82  & 8.73  & 89.61  & 2.84  & 3.04  & 93.40  \\ 
        (8 ,2 ,1 ,2)  & 21.35  & 21.69  & 98.41  & 16.16  & 15.96  & 98.76  & 7.82  & 8.64  & 90.57  & 2.64  & 3.12  & 84.45  \\ 
        (4 ,2 ,2 ,2)  & 22.68  & 22.57  & 99.52  & 16.50  & 16.16  & 97.93  & 8.82  & 9.03  & 97.66  & 2.64  & 2.94  & 89.69  \\ 
        (2 ,2 ,4 ,2)  & 24.70  & 23.83  & 96.38  & 17.18  & 16.80  & 97.78  & 10.16  & 9.67  & 95.00  & 2.64  & 3.03  & 87.41  \\ 
        (4 ,4 ,1 ,2)  & 22.19  & 24.11  & 92.03  & 17.27  & 16.75  & 96.89  & 7.74  & 9.74  & 79.46  & 2.82  & 2.70  & 95.78  \\ 
        (4 ,4 ,1 ,4)  & 21.97  & 24.15  & 91.00  & 17.00  & 16.91  & 99.42 & 7.74  & 9.92  & 78.03  & 2.78  & 2.91  & 95.21  \\ 
        (2 ,4 ,2 ,2)  & 23.80  & 24.97  & 95.30  & 17.63  & 17.07  & 96.72  & 8.98  & 9.98  & 89.99  & 2.82  & 2.70  & 95.45  \\ 
        (1 ,4 ,4 ,2)  & 26.15  & 26.28  & 99.52  & 18.36  & 17.74  & 96.52  & 10.61  & 10.51  & 99.05  & 2.82  & 2.87  & 98.33  \\ 
        (2 ,8 ,1 ,2)  & 24.75  & 26.61  & 93.03  & 19.89  & 19.90  & 99.97  & 8.10  & 9.48  & 85.50  & 3.25  & 3.21  & 98.89  \\ 
        (1 ,8 ,2 ,2)  & 27.06  & 28.12  & 96.23  & 20.31  & 20.16  & 99.22  & 9.99  & 9.99  & 99.99  & 3.25  & 3.24  & 99.95  \\ \hline
        \makecell{K coeff}  &   &   & 77\%  &   &   & 83\%  &  &  & 71\%  &   &   & 61\%  \\ \hline
    \end{tabular}
    \caption{Model accuracy evaluation result.}
    \label{acc_result}
\end{table*}
